Performance of Selection Combining for Differential Amplify-and-Forward Relaying Over Time-Varying Channels

Selection combining (SC) at the destination for differential amplify-and-forward (AF) relaying is attractive as it does not require channel state information as compared to the semi maximum-ratio-combining (semi-MRC) while delivering close performance. Performance analysis of the SC scheme was recently reported but only for the case of slow-fading channels. This paper provides an exact average bit-error-rate (BER) of the SC scheme over a general case of time-varying Rayleigh fading channels and when the DBPSK modulation is used together with the non-coherent detection at the destination. The presented analysis is thoroughly verified with simulation results in various fading scenarios. It is shown that the performance of the system is related to the auto-correlation values of the channels. It is also shown that the performance of the SC method is very close to that of the semi-MRC method and the existence of an error floor at high signal-to-noise ratio region is inevitable in both methods. The obtained BER analysis for the SC method can also be used to approximate the BER performance of the MRC method, whose exact analytical evaluation in time-varying channels appears to be difficult.

==> newcmd.tex <==
\newcommand{\dd}{{\mathrm d}}
\newcommand{\sd}{\mathrm{sd}}
\newcommand{\rd} {\mathrm{rd}}
\newcommand{\sr}{\mathrm{sr}}
\newcommand{\SC}{\mathrm{SC}}
\newcommand{\MRC}{\mathrm{MRC}}
\newcommand{\gth}{\gamma_{\mathrm{th}}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\CN}{\mathcal{CN}}
\newcommand{\Et}{\mathrm{E}}
\newcommand{\bt}{\mathrm{b}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\lpn}{\lim \limits_{P_0/N_0 \rightarrow \infty}}

